Currents and finite elements as tools for shape space

The nonlinear spaces of shapes (unparameterized immersed curves or submanifolds) are of interest for many applications in image analysis, such as the identification of shapes that are similar modulo the action of some group. In this paper we study a general representation of shapes that is based on linear spaces and is suitable for numerical discretization, being robust to noise. We develop the theory of currents for shape spaces by considering both the analytic and numerical aspects of the problem. In particular, we study the analytical properties of the current map and the $H^{-s}$ norm that it induces on shapes. We determine the conditions under which the current determines the shape. We then provide a finite element discretization of the currents that is a practical computational tool for shapes. Finally, we demonstrate this approach on a variety of examples.

==> frontmatter.tex <==
\newif\iffinal
\finalfalse
% \finaltrue

% -- Use utf-8 encoding for foreign characters
\usepackage[utf8]{inputenc}

\usepackage[l2tabu, orthodox]{nag}

\usepackage[left=2.5cm,top=2.5cm,right=2.5cm,bottom=2.5cm]{geometry}

% -- Color package
% \usepackage{tikz}
% \tikzset{>=stealth}
\usepackage[]{graphicx}
%\usepackage[rgb,dvipsnames]{xcolor}
\RequirePackage[svgnames]{xcolor}

%% -- Define mycolors
%\definecolor{mygreenc}{named}{OliveGreen}
%\definecolor{myredc}{named}{BrickRed}
%\definecolor{mybluec}{named}{NavyBlue}
%\definecolor{myorangec}{rgb}{1,0.4,0}
%\colorlet{myred}{myredc!70!black}
%\colorlet{myblue}{mybluec!50!black}
%\colorlet{mygreen}{mygreenc!70!black}
%\colorlet{myyellow}{yellow}
%\colorlet{myorange}{orange!50!white}
%% \colorlet{mygrey}{white!50!blue}
%\definecolor{mygrey}{rgb}{0.5,0.57,0.5}
%
%\colorlet{linkcolour}{green!40!black}
%\colorlet{urlcolour}{green!40!black}


% -- Hyperref package
\usepackage[pdfusetitle,pagebackref]{hyperref}
\hypersetup{
colorlinks=true,
linkcolor=DarkBlue,
citecolor=DarkGreen,
urlcolor=DarkMagenta,
  pdfauthor={James Benn, Stephen Marsland, Robert McLachlan, Klas Modin, Olivier Verdier},
	pdftitle={Shape currents}
}

% -- Various math packages
\usepackage{amsmath,amssymb}
\usepackage{aliascnt}
\usepackage{relsize} % Relative sizes: eg \smaller, \larger etc
\usepackage{enumitem}
\usepackage{mathtools}
\iffinal%
	\mathtoolsset{centercolon,showonlyrefs=false}
\else
	\mathtoolsset{centercolon,showonlyrefs=false}
\fi%

% -- Bibliography
\usepackage[numbers]{natbib} % Using \citet{...} for named citations.
\iffinal%
\else
	\usepackage[notref,notcite%
	]{showkeys}
	\usepackage{rotating}
	\renewcommand\showkeyslabelformat[1]{% 
	%\rotatebox{-90}{\normalfont\footnotesize\ttfamily\textcolor{cyan}{#1}}
	%\begin{turn}{-70}\normalfont\footnotesize\ttfamily\textcolor{myorange}{#1}\end{turn}%
	}
\fi%

% -- Fonts
\usepackage[T1]{fontenc}
%\usepackage{txfonts}
%\usepackage{mathrsfs}
%\usepackage{eucal}

% -- Todo notes
\usepackage[textsize=footnotesize,
\iffinal
disable,
\fi
]{todonotes}

\makeatletter 
\def\@seccntformat#1{\csname the#1\endcsname.\quad} 
\makeatother


\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{matrix}
\tikzstyle{commdiag}=[matrix of math nodes, row sep=3em, column sep=5.5em, text height=1.5ex, text depth=0.25ex,ampersand replacement=\&]
\tikzset{>=stealth}

\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\tikzstyle{none}=[inner sep=0pt]

% \usepackage{standalone}

% \usepackage{pgfplots}
% \pgfplotsset{compat=1.5.1}

% \usepackage{subfig}

% ------------------------------------------------------------------
% 		End: packages (end)
% ------------------------------------------------------------------


% ------------------------------------------------------------------
% 		Theorems, lemmas, etc and environments (fold)
% ------------------------------------------------------------------

% \usepackage{aliascnt}
% \usepackage{amsthm}
\newcommand{\newtheoremalias}[2]{%
\newaliascnt{#1}{theorem}%
\newtheorem{#1}[#1]{#2}%
\aliascntresetthe{#1}%
}

% \theoremstyle{plain}
%\newtheorem{theorem}{Theorem}[section]
%
%\newtheoremalias{proposition}{Proposition}
%\newcommand{\propositionautorefname}{Proposition}
%\newtheoremalias{corollary}{Corollary}
%\newcommand{\corollaryautorefname}{Corollary}
%\newtheoremalias{lemma}{Lemma}
%\newcommand{\lemmaautorefname}{Lemma}
%
%\theoremstyle{definition}
%\newtheoremalias{definition}{Definition}
%\newcommand{\definitionautorefname}{Definition}
%\newtheorem{assumption}{Assumption}
%\newcommand{\assumptionautorefname}{Assumption}
%\newtheorem{method}{Method}
%\newcommand{\methodautorefname}{Method}
%\newtheorem{algorithm}{Algorithm}
%\newcommand{\algorithmautorefname}{Algorithm}
%
%\theoremstyle{definition}
%\newtheoremalias{example}{Example}
%\newcommand{\exampleautorefname}{Example}
%\newtheoremalias{remark}{Remark}
%\newcommand{\remarkautorefname}{Remark}

\renewcommand*{\sectionautorefname}{Section}
\renewcommand*{\subsectionautorefname}{Section}
\renewcommand*{\subsubsectionautorefname}{\S\!}

\newcommand{\subfigureautorefname}{\figureautorefname}

% ------------------------------------------------------------------
% 		End: theorems (end)
% ------------------------------------------------------------------

% ------------------------------------------------------------------
% 		Title, author, etc (fold)
% ------------------------------------------------------------------

% -- Allows the command \affil{address etc} in the title page
\usepackage[affil-sl]{authblk} % affil-sl, affil-it, author-sl, author-it 
%\renewcommand\Authfont{\sffamily} 
\renewcommand\Affilfont{\slshape\small}


\title{Currents and finite elements as tools for shape space}
\author{James Benn \and Stephen Marsland \and Robert I McLachlan \and Klas Modin \and Olivier Verdier}
\institute{JB \at 3 Hardie Street, Palmerston North, New Zealand\\ \email{jbenn2@alumni.nd.edu} 
\and SM \at School of Mathematics and Statistics, Victoria University of Wellington, New Zealand\\  \email{stephen.marsland@vuw.ac.nz}. Phone: +64 4 463 9695.
\and RIM \at Institute of Fundamental Sciences, Massey University, New Zealand\\  \email{r.mclachlan@massey.ac.nz}
\and KM \at Department of Mathematical Sciences, Chalmers University of Technology and University of Gothenburg, Sweden\\ \email{klas.modin@chalmers.se}
\and OV \at Department of Computing, Mathematics and Physics, Western Norway University of Applied Sciences, Bergen, Norway and Department of Mathematics, KTH, Stockholm, Sweden\\ \email{olivier.verdier@hvl.no, olivierv@kth.se}
}

\date{Received: date / Accepted: date}

% ------------------------------------------------------------------
% 		End: title (end)
% ------------------------------------------------------------------

% ------------------------------------------------------------------
% 		Definitions (fold)
% ------------------------------------------------------------------


